Online Clique Clustering

Clique clustering is the problem of partitioning the vertices of a graph into disjoint clusters, where each cluster forms a clique in the graph, while optimizing some objective function. In online clustering, the input graph is given one vertex at a time, and any vertices that have previously been clustered together are not allowed to be separated. The goal is to maintain a clustering with an objective value close to the optimal solution. For the variant where we want to maximize the number of edges in the clusters, we propose an online strategy based on the doubling technique. It has an asymptotic competitive ratio at most 15.646 and an absolute competitive ratio at most 22.641. We also show that no deterministic strategy can have an asymptotic competitive ratio better than 6. For the variant where we want to minimize the number of edges between clusters, we show that the deterministic competitive ratio of the problem is $n-\omega(1)$, where n is the number of vertices in the graph.

==> binom_lemma.tex <==


%%%%%%%%%%%%%

\begin{lemma}\label{lem:profvalue}
For any pair of non-negative integers $a$ and $b$, the inequality 
%
{\small
\begin{equation*}
\profvalue{a+b} \leq (x+1)\profvalue{a} + \frac{x+1}{x}\profvalue{b} + a
\end{equation*}
}
%
holds for any $0<x\leq1$.
\end{lemma}

\begin{proof}
Define the function
%{\small
\begin{align*}
F(a,b,x) & = 2x(x+1)\profvalue{a} + 2(x+1)\profvalue{b} + 2ax - 2x\profvalue{a+b}
\\
& = 
a^2x^2 - ax^2 + 2ax + b^2 - b - 2abx
 =
(b-ax)^2 + ax(2-x) - b,
\end{align*}
%}
i.e., twice $x$ times the difference between the right hand side and the left hand side of the inequality above.
%
It is sufficient to show that $F(a,b,x)$ is non-negative for integers $a,b\geq0$ and $0<x\leq1$.

Consider first the cases when $a\in \{0,1\}$ or $b\in\{0,1\}$.
$F(0,b,x)=b(b-1)\geq0$, for any non-negative integer $b$ and any~$x$.
$F(a,0,x)=ax(ax-x+2)\geq ax(ax+1)>0$, for any positive integer $a$ and $0<x\leq1$.
$F(a,1,x)=x^2a(a-1)\geq0$, for any positive integer $a$ and any~$x$.
$F(1,2,x)=2-2x\geq0$, for $0<x\leq1$, and $F(1,b,x)=b^2-b+2x-2bx\geq b^2-3b\geq0$, for any integer $b\geq3$ and $0<x\leq1$.

Thus, it only remains to show that $F(a,b,x)$ is non-negative when both $a\geq2$ and~$b\geq2$.
The function $F(a,b,x)$ is quadratic and hence has one local minimum at $x_0=\frac{b-1}{a-1}$, 
as can be easily verified by differentiating $F$ in~$x$.
Therefore, in the case when $a\leq b$, $F(a,b,x)\geq F(a,b,1)=(b-a)^2 - (b-a)\geq(b-a) - (b-a)=0$, for $0<x\leq1$.
In the case when $a>b$, we have that $F(a,b,x)\geq F(a,b,\frac{b-1}{a-1})=\frac{(a-b)(b-1)}{a-1}>0$, which completes the proof.
%\hfill$\Box$
\end{proof}


==> maxclustering.tex <==

%\section{Online Maximum Clique Clustering}
%\label{sec: maxclustering}
%\input{maxclustering.tex}

\subsection{The Greedy Strategy for Online Max-CC}\label{subsec:maxgreedy}

The {\em greedy\/} strategy for Max-CC merges each input vertex with the largest current cluster that maintains the clique property. If no such merging is possible the vertex is placed in a singleton cluster. Greedy strategies are natural first attempts used to solve online problems and can be shown to behave well for certain of them; e.g.~\cite{MathieuSS_correlation_2010}. We show that the greedy strategy can be far from optimal for Max-CC.

\begin{theorem}\label{thm:maxgreedylowerbound}
The greedy strategy for Max-CC is no better than $(n-2)/2$-competitive.
\end{theorem}
\begin{proof}
Consider an adversary that provides input to the strategy to make it behave as badly as possible. Our adversary gives greedy $n=2k$ vertices in order from 1 to $2k$. Each odd numbered vertex is connected to its even successor, each odd numbered vertex is also connected to every other odd numbered vertex before it, and similarly, each even numbered vertex is also connected to every even numbered vertex before it, thus defining the graph $G$; see Figure~\ref{fig:greedyex}.
\begin{figure}[htb]
\begin{center}
\includegraphics{Figures/fig2.pdf}
%\caption{\label{figma} Each odd numbered vertex is connected to its even successor, each odd numbered vertex is connected to every odd numbered vertex before it and each even numbered vertex is also connected to each even numbered vertex before it.}
\caption{\label{fig:greedyex}Illustrating the proof of Theorem~\protect\ref{thm:maxgreedylowerbound}.}
\end{center}
\end{figure}%\vspace*{-6ex}

The greedy strategy clusters the vertices as odd/even pairs, giving a clustering having profit $\profit_{\GDY}(G)=k$. An optimal strategy clusters the odd vertices in one clique of size $k$ and the even vertices in another clique also of size $k$. The profit for the optimal solution is $\profit_{\opt}(G)=k(k-1)$. Hence, the worst case ratio between an optimum and a greedy solution is at least $k-1=n/2-1$ so the competitive ratio is at least~$(n-2)/2$.
%\hfill$\Box$
\end{proof}

Next, we look at the upper bound for the greedy strategy.
\begin{theorem}\label{thm:maxgreedyupperbound}
The greedy strategy for Max-CC is $(n-2)$-competitive.
\end{theorem}
\begin{proof}
Consider an edge $e$ inside a cluster produced by the greedy strategy on $n$ vertices of $G$. We introduce a weight function $w(e)$ as follows: fix an optimal clustering on $G$ that we denote $\OPT(G)$. If $e$ also belongs to a cluster in $\OPT(G)$, then we set $w(e)\defeq1$. If $e$ does not belong to any cluster in $\OPT(G)$, then the two endpoints $v$ and $v'$ belong to different clusters of $\OPT(G)$. Denote these two clusters by $c_e$ and $c'_e$ and we set $w(e)\defeq|c_e|+|c'_e|-2$, i.e., the number of edges in $c_e$ and $c'_e$ connected to $v$ and~$v'$. Note that not both $c_e$ and $c'_e$ can be singleton clusters, so $w(e)\geq1$ for every edge $e$ in~$G$.

Consider now the sum, $\sum_{e\in\GDY(G)}w(e)$, where we let $e\in\GDY(G)$ denote that two end points of edge $e$ lie in the same cluster of $\GDY(G)$, the greedy clustering on~$G$. The sum counts every edge in $\OPT(G)$ at least once, since an edge lying inside clusters of both $\GDY(G)$ and $\OPT(G)$ is counted once and an edge lying in a cluster of $\GDY(G)$ but outside all clusters of $\OPT(G)$ counts all the edges in clusters of $\OPT(G)$ that are connected to the two endpoints. The fact that the sum counts all the edges in clusters of $\OPT(G)$ follows since no two clusters in greedy can be merged to a single cluster. Hence,
\begin{eqnarray*}
\opt(G) & \leq & \sum_{e\in\GDY(G)} w(e) \leq \sum_{e\in\GDY(G)} |c_e|+|c'_e|-2 
\leq (|c_1|+|c_2|-2)\cdot\sum_{e\in\GDY(G)} 1 
\\& \leq &  (|c_1|+|c_2|-2)\cdot \profit_{\GDY}(G) \leq (n-2)\cdot \profit_{\GDY}(G),
\end{eqnarray*}
where $c_1$ and $c_2$ denote the two largest clusters in~$\OPT(G)$.
%\hfill$\Box$
\end{proof}

